VIP Hashing -- Adapting to Skew in Popularity of Data on the Fly (extended version)

All data is not equally popular. Often, some portion of data is more frequently accessed than the rest, which causes a skew in popularity of the data items. Adapting to this skew can improve performance, and this topic has been studied extensively in the past for disk-based settings. In this work, we consider an in-memory data structure, namely hash table, and show how one can leverage the skew in popularity for higher performance. Hashing is a low-latency operation, sensitive to the effects of caching, branch prediction, and code complexity among other factors. These factors make learning in-the-loop especially challenging as the overhead of performing any additional operations can be significant. In this paper, we propose VIP hashing, a fully online hash table method, that uses lightweight mechanisms for learning the skew in popularity and adapting the hash table layout. These mechanisms are non-blocking, and their overhead is controlled by sensing changes in the popularity distribution to dynamically switch-on/off the learning mechanism as needed. We tested VIP hashing against a variety of workloads generated by Wiscer, a homegrown hashing measurement tool, and find that it improves performance in the presence of skew (22% increase in fetch operation throughput for a hash table with one million keys under low skew, 77% increase under medium skew) while being robust to insert and delete operations, and changing popularity distribution of keys. We find that VIP hashing reduces the end-to-end execution time of TPC-H query 9, which is the most expensive TPC-H query, by 20% under medium skew.

==> sections/conclusions.tex <==
\revision{In conclusion, we have shown that optimizing a database engine for a particular SSD can be beneficial. Our contributions are threefold; \textit{learning} hidden parameters of SSDs (\S\ref{learn}), proposing \textit{rules} specific to a device (\S\ref{observe}), and \textit{optimizing} database engines for the device using these rules (\S\ref{propose}). We have studied SQLite3 and MariaDB as part of our work, and we propose three techniques to optimize these database engines, namely \textit{use-hot-locations} (Fig.~\ref{fig:use-good-locations}), \textit{write-aligned-stripes} (Fig.~\ref{fig:write-stripes}), and \textit{contain-write-in-flash-page} (Fig.~\ref{fig:contain-write-in-flash-page}). These techniques increased the throughput of select operations by 27-29\% on SSD-S, and reduced the wear-out caused to SSD-T by 3.1\% and 6.7\% respectively.}

%We obtain two different characteristics of an SSD, namely the \textit{request size profile} and the \textit{location profile}, from which we learn multiple internal parameters. Based on these internal parameters, we propose rules to analyze the I/O behavior of a database engine. Using these rules, we uncover sub-optimal I/O patterns in SQLite3 and MariaDB when running on our experimental SSDs. Finally, we present three techniques for optimizing these database engines: (1) \textit{use-hot-locations} on SSD-S, which improves the SELECT operation throughput of SQLite3 and MariaDB by 29\% and 27\% respectively; it also improves the performance of YCSB on MariaDB by 3\%-46\% depending on the workload mix used, (2) \textit{write-aligned-stripes} on SSD-T, reduces the wear-out caused by SQLite3 write-ahead log (WAL) file by 3.1\%, and (3) \textit{contain-write-in-flash-page} on SSD-T, which reduces the wear-out caused by the MariaDB binary log file by 6.7\%.

\revision{As future work, it is possible to implement the proposed rules and techniques in an independent pluggable layer for applications to use. We envision this layer to be highly configurable, as often applications have the broader view of their performance goals and some corrections (eg. \textit{write-aligned-stripes}) can be best made by them.} Overall, SSDs are complex devices with a range of characteristics. We would like to reiterate that there is no silver bullet to learn all the internal parameters of every SSD. However, we believe that such an attempt is worthwhile, and we have found that besides benefiting the database engine they can improve the expected performance and the lifetime of the SSD as well. The parameters learned and the recommendations outlined in this paper are by no means complete, and the most reliable source of this information are vendors themselves. Thus, we would like to end with a recommendation for SSD manufacturers to be more transparent regarding basic parameters such as the flash page size and the stripe size.

==> sections/optimizing_dbms.tex <==
In this section, we describe our approach towards optimizing databases for an SSD. We first measure the SSD's characteristics and learn some internal parameters (\S\ref{learn}). Informed by these parameters, we describe rules to identify any sub-optimal I/O requests issued by the database engine (\S\ref{observe}). Finally, we propose techniques to eliminate these sub-optimal I/O requests, and improve the performance of the database engine on the SSD (\S\ref{propose}). {The SSDs used for experiments in this section, as well as their parameters learned have been summarized in Table \ref{ssds}. SSD-S, SSD-T, and SSD-M are NAND flash based, whereas SSD-I is built with 3D XPoint memory.}

% There are three steps to optimizing a database engine for an SSD. First, we learn the unique internal characteristics of an SSD through various experiments (\S\ref{learn}). Next, we observe the I/O patterns of the database engine using \textit{blktrace} (\S\ref{observe}). Finally, we propose rules for improving performance by considering the properties of the SSD and the database engine (\S\ref{propose}).

% \subsection{The Request Size Profile of an SSD}

% \subsubsection{Learning the SSD Stripe Size}

% \subsection{The Location Profile of an SSD}

% \subsection{Observing I/O patterns}

% \subsection{Proposing Rules to Improve Performance?}

\subsection{Learning SSD Parameters}\label{learn}

% The physical layout policy of the FTL plays a key role in determining an SSD's performance, and this knowledge can be helpful in effectively utilizing the device. 

We study two types of characteristics of an SSD, which help us infer various internal parameters. First, we describe how to obtain the \textit{request size profile} (\S\ref{request-size-profile}), from which we learn the \textit{desirable write request sizes} and the \textit{stripe size} of an SSD. \revision{Next, we obtain the \textit{location profile} (\S\ref{location-profile}) of the SSDs, from which we identify their respective \textit{chunk sizes}, \textit{hot locations}, and \textit{flash page sizes}.}

% The physical layout policy of the FTL plays a key role in determining an SSD's performance, and this knowledge can be helpful in effectively utilizing the device. We study two types of characteristics of an SSD, namely the \textit{request size profile} (\S\ref{request-size-profile}) and the \textit{location profile} (\S\ref{location-profile}), which help us obtain various parameters of an SSD.

% The request size profile helps us learn the \textit{recommended write sizes} and the \textit{stripe size} of an SSD. Next, we obtain the \textit{location profile} of all the SSDs, which helps us identify the \textit{chunk size} and \textit{hot locations} in the logical address space.

% We study two characteristics of SSDs, namely the \textit{request size profile} (\S\ref{request-size-profile}) and the \textit{location profile} (\S\ref{location-profile}), which we use to learn parameters unique to an SSD. We discuss how to find an SSD's \textit{stripe size}, \textit{recommended write sizes}, and \textit{hot locations} from these measurements. 

% \begin{table*}
% 	\centering
% 	\caption{SSDs used in experiments}
% 	\begin{tabular}{|c|c|c|c|c|c|c|c|} \hline
% 		\textbf{Label} & \textbf{Name} & \textbf{Capacity} & \textbf{Interface}\\ \hline
% 		SSD-S & Samsung 960 EVO & 512GB & NVMe / PCIe\\ \hline
% 		SSD-I & Intel Optane 905P & 480 & NVMe / PCIe\\ \hline
% 		SSD-T & Toshiba XG5 &  256GB & NVMe / PCIe\\
% 		\hline
% 		SSD-M & Micron M500 &  120GB & SATA\\
% 		\hline
% 	\end{tabular}
% 	\label{ssds}
% \end{table*}

% There is a strong correlation between the latency of a request and the physical layout of data. To motivate this, consider three requests of the same size as shown in Fig. \ref{physical-location-imp}. These requests can have significantly different latencies depending on the \textit{amount of data accessed internally} for the request, and the \textit{utilization of internal parallelism}. A request aligned with a flash page (Fig. \ref{single-page}) accessing fewer flash pages, and a request which utilizes channel-level parallelism (Fig. \ref{different-channel}) will be both be faster compared to an unaligned non-parallel request (Fig. \ref{same-channel}). Thus, the knowledge of the physical layout can potentially benefit an application.

% This is for removing space after the algorithms
% This location is very hackily chosen
% Remove this if it doesn't work
\setlength{\textfloatsep}{4pt}
\begin{algorithm}
	\caption{The Location Profile of an SSD}\label{exp-location-profile}
	\begin{algorithmic}[1]
		\Procedure{GetLocationProfile}{}
		\State \textit{filename} $\gets$ \textit{512KB-seq}
		\State \textit{file} $\gets open(filename)$
		\State $fileSize \gets 1GB$
		\State $chunkSizeMin \gets 4KB$
		\State $chunkSizeMax \gets 512KB$
		\State \textit{offsetUnit} $\gets 1KB$
		\State $expChunkSize \gets chunkSizeMin$
		\While{$expChunkSize <= chunkSizeMax$}
		\State \textit{numChunks} $\gets$ \textit{fileSize/expChunkSize}
		\State \textit{randChunks} $\gets$ \textit{random\_shuffle(1:numChunks)}
		\State \textit{numOffsetGroups} $\gets$ \textit{chunkSize/offsetUnit}
		\For{\textit{i} \textbf{in} \textit{0:(numOffsetGroups-1)}}
		\State \textit{latencies} $\gets []$
		\For{\textit{j} \textbf{in} \textit{randChunks}}
		\State \textit{chunkOffset}$ \gets (j-1)\times chunkSize$
		\State \textit{offset} $\gets$\textit{chunkOffset}$ + i\times$ \textit{offsetUnit}
		\State \textit{startTime} $\gets time.now()$
		\State \textit{data} $\gets read(file, chunkSize, $\textit{offset)}
		\State \textit{endTime} $\gets time.now()$
		\State \textit{latencies.append($endTime-startTime$)}
		\EndFor
		\State \textit{plot(expChunkSize, latencies, offsetGroup=i)}
		\EndFor
		\State $expChunkSize \gets 2\times expChunkSize$
		\EndWhile
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

\subsubsection{The Request Size Profile}\label{request-size-profile}

Experiment \ref{exp-request-size-profile} describes how to obtain the request size profile of an SSD. We start by creating files of size 1GB with sequential write requests of sizes ranging from 1KB to 512KB (filename \textit{512kb-seq} refers to a 1GB file created with sequential write requests of size 512KB; likewise for other request sizes). Following this, the latency of read requests to all the files is measured. This experiment helps determine which write request sizes are desirable for a given SSD; a higher latency of read requests indicates an undesirable write request size during file creation.

Fig. \ref{request-size-profile-ssds} shows the request size profile of all the SSDs, and we find that different devices have different characteristics. For a given SSD, we identify the request size at which minimum latency is attained, and all sizes greater than that, as \textit{desirable write request sizes}. Two factors contribute to higher latency of a read request, namely read/write amplification and higher address translation time. The request size at which the lowest latency is obtained suggests absence of these factors, and is thus desirable. Thus, for SSD-S, request sizes 32KB and above are desirable, whereas for SSD-T and SSD-M, the desirable request sizes are 64KB and above.

%  For SSD-S, SSD-T and SSD-C, we observe that minimum latency is attained at write requests of sizes 32KB, 64KB, and 8KB respectively. Discuss results

%   The FTL decides the physical layout of data for a write request, and this is likely to vary for different request sizes.

% The concept of stripe size is generic, and does not assume any structure to the physical storage format.

%  Conversely, this suggests that the number of sub-units is dependent on the stripe size of the SSD. The number of sub-units spanned over determines the internal parallelism utilized by a request. This is the motivation behind our first experiment for learning the stripe size (Exp. \ref{exp-request-size-profile}).

% In the experiment (Exp. \ref{exp-request-size-profile}), we create ten different files of size 1GB with increasing experimental stripe sizes ranging from 1KB to 512KB. The aim of the experiment is to find the experimental stripe size that matches the internal stripe size of the SSD. Each file created in the experiment is named appropriately, where \textit{1KB-seq} denotes the file created with an experimental stripe size of 1KB, with stripes of data written in a sequential order.

% After creating the files, we issue read requests of size 512KB to all aligned offsets in a random order (total 2K requests to each file). We record and plot the latency of requests and compare results from all the files.

% Through this experiment, our aim is to analyze the physical layout of different files, which we achieve by comparing the latency of requests to them. In all cases, the latency becomes nearly constant after a certain experimental stripe size. This suggests that the internal physical layout of all these files is similar, indicating that the stripe size at which the curve becomes constant is the internal stripe size. We find that SSD-S and SSD-T have a stripe size of 64KB, whereas SSD-I and SSD-C have 4KB and 8KB stripes respectively. 
	
Next, we attempt to learn the \textit{stripe size} of the SSDs. We define the stripe size as the unit of decision of physical layout inside an SSD. Two (aligned) stripes of data have similar layout in terms of the sub-units occupied at each level of the flash hierarchy. The latency of read requests depends on the internal parallelism utilized inside the SSD, which in turn depends on the physical layout of data. Thus, similar latency of read requests indicates a similarity in physical layout of data. Therefore, for SSD-T, files \textit{64kb-seq} to \textit{512kb-seq} have similar physical layout, indicating that 64KB is the stripe size. By a similar argument, the stripe size of SSD-S and SSD-M is also 64KB.

\begin{figure*}
	\centering
	\subfloat[SSD-S. Request sizes 32KB and up are desirable. The latency becomes roughly constant after request size 64KB, indicating that it is the stripe size.]{
		\includegraphics[scale=0.35]{figures/samsung_stripes.png}
		\label{samsung-stripes}
	}
	\hspace{3mm}
	\subfloat[SSD-T. Request sizes 64KB and up are desirable. The latency becomes roughly constant after request size 64KB, indicating that it is the stripe size.]{
		\includegraphics[scale=0.35]{figures/toshiba_stripes.png}
		\label{same-channel}
	}
	
	\vspace{-0.4em}
	\subfloat[SSD-I. All request sizes are desirable. This experiment is insufficient to learn the stripe size of this SSD.]{
		\includegraphics[scale=0.35]{figures/optane_stripes.png}
		\label{different-channel}
	}
	\hspace{3mm}
	\subfloat[SSD-M. Request sizes 64KB and up are desirable. The latency becomes roughly constant after request size 64KB, indicating that it is the stripe size.]{
		\includegraphics[scale=0.35]{figures/micron_stripes.png}
		\label{different-channel}
	}
	\vspace{-.4em}
	\caption{\textbf{The Request Size Profile. We learn the \textit{stripe size} and \textit{desirable request sizes} from Experiment \ref{exp-request-size-profile}.}}
%		\vspace{-1em}
	\label{request-size-profile-ssds}
\end{figure*}

% The physical layout of data is determined by the FTL at the time of file creation. The latency of a subsequent read request depends on the amount of internal parallelism utilized inside the SSD (which in turn depends on the physical layout). Thus, differences in physical layout of data are reflected through differences in latency of read requests.

% Conversely, similar latency of read requests indicates similarity in physical layout of data. SSDs often use RAID like schemes~\cite{} where data is striped and laid out over sub-units at different levels of flash storage (over channels, packages, chips, and planes).  We define the \textit{stripe size} as the unit of decision for the physical layout inside an SSD.

% For SSD-S, we find that the latency of read requests becomes almost constant after a write request size of 64KB. This indicates that all of these files have the same physical layout. Thus, a write request of 64KB equals the internal stripe size for SSD-S. By a similar argument, we find that the stripe size of SSD-M and SSD-T is also 64KB.

Unlike the others, SSD-I has constant latency for all the files. Flash-based SSDs can incur read/write amplification, as flash pages are units of read/write operations. However, unlike flash memory, Intel's 3D XPoint memory is byte-addressable and need not be erased before overwriting, and this is perhaps the reason behind the difference in SSD-I's behavior. Although we find that none of the request sizes are particularly undesirable for SSD-I, this experiment is insufficient to learn its stripe size.

% Unlike the others, SSD-I has constant latency for all the files. In the case of flash SSDs, the flash page is the unit of write requests. Any requests smaller than flash page size needs to be padded up, causing write amplification (and also \textit{read amplification} for subsequent read requests as more flash pages than necessary need to be accessed). This property of flash memory does not hold true for Intel's 3D XPoint memory, which is byte-addressable, and is perhaps the reason behind the difference in the behavior. Although we find that none of the request sizes are particularly undesirable for SSD-I, this experiment is insufficient to learn the stripe size of SSD-I.

% Unlike other SSDs, SSD-I has a constant latency for all the files. SSD-I is built with 3D XPoint memory, which is byte-addressable and need not be overwritten. 

\subsubsection{The Location Profile}\label{location-profile}

\begin{figure}
	\centering
	\subfloat[An example of an 8KB write request to an SSD with chunk size 4KB. Two chunks of 4KB are stored on each channel.]{
		\includegraphics[scale=0.18]{figures/Write-0-16kb.pdf}
		\label{write-0-8kb}
	}
	\hspace{1.5mm}
	\subfloat[A 4KB read request aligning with a chunk; data on Channel \#0 alone is accessed.]{
		\includegraphics[scale=0.18]{figures/Read-0-8kb.pdf}
		\label{read-0-4kb}
	}
	
	\vspace{-0.4em}
	\subfloat[A 4KB read request offset into a chunk. If the flash page size is 2KB, required pages are accessed in parallel, which will be faster than Fig. \ref{read-0-4kb}.]{
		\includegraphics[scale=0.18]{figures/Read-4-12kb-good.pdf}
		\label{read-2-6kb-good}
	}
	\hspace{1.5mm}
	\subfloat[A 4KB read request offset into a chunk. If the flash page size is 4KB, both the chunks(pages) will be fetched. Will be slower than Fig. \ref{read-0-4kb}.]{
		\includegraphics[scale=0.18]{figures/Read-4-12kb-bad.pdf}
		\label{read-2-6kb-bad}
	}
	\vspace{-0.4em}
	\caption{\textbf{Impact of channel-level parallelism on the latency of read requests at different logical address locations. If the flash page size is smaller than the chunk size, channel-level parallelism reduces latency by doubling the bandwidth (Fig. \ref{read-2-6kb-good}). Otherwise, it increases latency due to read amplification (Fig.\ref{read-2-6kb-bad}).}}
	\label{physical-location-imp}
\end{figure}

%\begin{figure*}
%	\centering
%	\subfloat[SSD-S. Latency of read requests at offset group 32KB is 39\% lower than offset group 0. The chunk size is 64KB, and the hot locations are at offset group 32KB.]{
%		\includegraphics[scale=0.35]{figures/samsung_loc.png}
%		\label{fig:samsung-loc}
%	}
%	\hspace{2mm}
%	\subfloat[SSD-T. Latency of read requests at offset group 0 is 38\% lower compared to others. The chunk size is 4KB, and the hot locations are at offset group 0.]{
%		\includegraphics[scale=0.35]{figures/toshiba_loc.png}
%		\label{fig:toshiba-loc}
%	}
%	
%	\subfloat[SSD-I. Latency of read requests at offset group 0 is 9\% lower compared to others. The chunk size is 4KB, and the hot locations are at offset group 0.]{
%		\includegraphics[scale=0.35]{figures/optane_loc.png}
%		\label{fig:optane-loc}
%	}
%	\hspace{2mm}
%	\subfloat[SSD-M. Latency of read requests at offset group 0 is 20\% lower compared to others. The chunk size is 4KB, and the hot locations are at offset group 0.]{
%		\includegraphics[scale=0.35]{figures/micron_loc.png}
%		\label{fig:micron-loc}
%	}
%	\caption{\textbf{The Location Profile. We learn the \textit{chunk size} and \textit{hot locations} of all the SSDs from Experiment \ref{exp-location-profile}.}}
%	\label{location-profile-exp}
%\end{figure*}
\begin{figure*}
	\centering
	\subfloat[{\textbf{SSD-S}. Latency of reads at offset group 32KB is 39\% lower than offset at group 0. The chunk size is 64KB, and the hot locations are at offset group 32KB.}]{
		\includegraphics[scale=0.35]{figures/samsung_loc_new.png}
		\label{fig:samsung-loc}
	}
	\hspace{1.5mm}
	\subfloat[{\textbf{SSD-T}. Latency of read requests at offset group 0 is 38\% lower compared to others. The chunk size is 4KB, and the hot locations are at offset group 0.}]{
		\includegraphics[scale=0.35]{figures/toshiba_loc_new.png}
		\label{fig:toshiba-loc}
	}
	\hspace{1.5mm}
	\subfloat[{\textbf{SSD-I}. Latency of read requests at offset group 0 is 9\% lower compared to others. The chunk size is 4KB, and the hot locations are at offset group 0.}]{
		\includegraphics[scale=0.35]{figures/optane_loc_new.png}
		\label{fig:optane-loc}
	}
	\hspace{1.5mm}
	\subfloat[{\textbf{SSD-M}. Latency of read requests at offset group 0 is 20\% lower compared to others. The chunk size is 4KB, and the hot locations are at offset group 0.}]{
		\includegraphics[scale=0.35]{figures/micron_loc_new.png}
		\label{fig:micron-loc}
	}
	\vspace{-0.4em}
	\caption{\textbf{The Location Profile. We learn the \textit{chunk size} and \textit{hot locations} of the SSDs from Experiment \ref{exp-location-profile}.}}
	\label{location-profile-exp}
\end{figure*}
% \begin{figure*}
% \centering
% \subfloat[Fetching a single flash page for an 8KB read request.]{
% 	\includegraphics[scale=0.21]{read_0_8kb.pdf}
%     \label{single-page}
% }
% \hspace{3mm}
% \subfloat[Fetching two flash pages from the same flash package. Does not utilize channel-level parallelism. ]{
% 	\includegraphics[scale=0.21]{read_4_12kb_same_package.pdf}
%     \label{same-channel}
% }
% \hspace{3mm}
% \subfloat[Fetching two flash pages on different channels. Utilizes channel-level parallelism.]{
% 	\includegraphics[scale=0.21]{read_4_12KB.pdf}
%     \label{different-channel}
% }
% \caption{\textbf{The importance of physical layout for performance. A request of size 8KB is issued in each case. The request in (a) fetches a single flash page, and will be faster than (b). The request in (c) utilizes channel-level parallelism, and will also be faster than (b). The difference between (a) and (c) might be negligible, if both the flash pages are fetched concurrently in (c). (TODO: Fix this fig)}}
% \label{physical-location-imp}
% \end{figure*}
%Having found the stripe size, we can use this information to further study how stripes are physically laid out inside the SSD. Our next experiment (Exp. \ref{exp2}) attempts to learn how two consecutive stripes are stored relative to each other~\cite{}. Some filler sentence.

We define the \textit{chunk size} of an SSD as the amount of contiguous data stored on a single channel. Due to the hierarchical architecture of SSDs, the latency of read requests (of chunk size) can vary at different logical address locations. Fig. \ref{physical-location-imp} shows the multiple cases that can arise. If a request internally spans over multiple channels, its latency can be relatively lower or higher depending on the flash page size and chunk size of the SSD. This is the motivation behind Experiment \ref{exp-location-profile}, which is inspired by Chen et al.~\cite{EssentialRoles}.

In the experiment, we repeatedly guess a chunk size and issue read requests (of chunk size) at different logical address locations, giving rise to the location profile of an SSD (for that chunk size). We define an \textit{offset group} as the group of logical addresses with the same relative offset into a chunk\footnote{For example, offset group 1KB for chunk size 4KB refers to all logical address locations of the form 4KB$\times i +$1KB.}. If a significant variation in latency between different offset groups is observed, it indicates an influence of channel-level parallelism in some form.

Fig. \ref{location-profile-exp} shows the result of this experiment. For SSD-S, we observe that for a chunk size of 64KB, offset group 32KB has 39\% lower latency than offset group 0. Thus, the 32KB location group constitutes the set of \textit{hot locations} on SSD-S. This behavior is similar to Fig. \ref{read-2-6kb-good}, where channel-level parallelism helps reduce latency. \revision{On the other hand, the remaining SSDs have behavior similar to Fig. \ref{read-2-6kb-bad} with minimum latency at offset group 0, with a flash page size and chunk size of 4KB}. We find that the reduction in latency at hot locations varies from one device to another, and this has been reported in Fig. \ref{location-profile-exp}.

% This is for removing space after the algorithms
% This location is very hackily chosen
% Remove this if it doesn't work
\setlength{\textfloatsep}{\textfloatsepsave}
%	The benefit of hot locations for the SSDs has been reported in Fig. \ref{location-profile-exp}, and varies from one device to another.


% Having found the stripe size, the next question that arises is how stripes are laid out physically. Do two consecutive stripes share the same physical sub-units? If two stripes are placed on different internal channels, then there is scope for utilizing channel-level parallelism at the application level. Channels are the first level of the flash storage hierarchy, and have the most influence on the latency of a request. Our next experiment (Exp. \ref{exp2}) borrowed from previous work~\cite{} attempts to learn if two consecutive stripes share common sub-units.

%Channels are the first level of the flash storage hierarchy, and among all levels, channel-level parallelism has the most impact on the latency of a request (Fig. \ref{physical-location-imp}). This also means that channel-level contention is most discernible from the latency of requests.

% Figure \ref{location-profile-exp} shows the result of this experiment. We define an \textit{offset group} as the group of addresses with the same relative offset into a stripe (for example, offset group $0$ denotes all read requests aligning with a stripe boundary). For SSD-S, we find that the latency at offset group 32KB is 42\% lower than the latency at offset group 0. On the other hand, for SSD-M, the latency at offset group 0 is 29\% lower than the others. Thus, offset group 32KB and 0KB are "good locations" for SSD-S and SSD-M respectively.

% In the case of SSD-I, we were unable to determine the stripe size from Experiment \ref{exp-request-size-profile}. Thus, we guess a stripe size before performing Experiment 2. We find that for a stripe size of 4KB, we observe a 12\% difference in latency between offset group 0 and 3KB. This result is also corroborated by previous work~\cite{}, which mentions that 4KB of data is stored on a channel inside SSD-I. For SSD-T, we do not observe any difference in latency at different offset groups. This is perhaps because of a behavior similar to Figure \ref{}. Thus, there are no good locations
% on SSD-T. <-- Need to re-check this again.

% Should I also talk about different request sizes having a different set of good locations? Perhaps this can be interesting. Can talk about 32KB requests on SSD-S.

% In the experiment (Exp. \ref{exp2}), we issue read requests equal to the stripe size at different offsets in a file. We define an \textit{offset group} as the group of addresses with the same relative offset into a stripe (for example, offset group $0$ denotes all read requests aligning with a stripe boundary). We measure and plot the latency of all read requests at each offset group. Fig. \ref{location-profile-exp} shows the result of this experiment for all the SSDs.

%	Introducing Rules to Analyze I/O Patterns

\subsection{Rules to Analyze Database I/O Patterns}\label{observe}

In the previous section, we described how to learn some internal parameters of an SSD. In this section, we use these parameters to propose rules for applications when running on a given SSD (\S\ref{identify-io-calls}).

%These rules can be used to find an application's sub-optimal I/O patterns when running on a particular SSD.

% In this section, we use these parameters to propose rules specific to an SSD (\S\ref{identify-io-calls}). By following these rules, applications can maximize the performance obtained from the SSD and/or increase its lifetime.

We first run a benchmark experiment (\S\ref{benchmark-exp}) to obtain the I/O patterns of a database engine, followed by applying the rules to analyze the I/O requests (\S\ref{analyzing-btree} and \S\ref{analyzing-logs}). Requests that violate the rules are considered sub-optimal, and identifying such requests reveals opportunities for improving the performance of a database engine on a particular SSD. \revision{Thus, by using this approach, we study SQLite3 and MariaDB on two of our experimental SSDs, namely SSD-S and SSD-T, and we find sub-optimal I/O patterns in both of these database engines.}

%\revision{Thus, by using this approach, we find sub-optimal I/O patterns in our test database engines, namely SQLite3 and MariaDB, on two of our experimental SSDs: SSD-S and SSD-T.}

% We give an example of using these rules by applying them to SQLite3. To record the read/write I/O patterns of SQLite3, we first run a benchmark experiment (\S\ref{benchmark-exp}). Finally, we analyze the I/O calls and identify the requests that violate the described rules (\S\ref{analyzing-sqlite3}).

% We describe a benchmark experiment (\S\ref{benchmark-exp}) and record the read/write I/O requests issued by a database engine using \textit{strace}~\cite{}. Finally, we apply these rules to analyze the I/O patterns of SQLite3 (\S\ref{analyzing-sqlite3}).

\subsubsection{Rules to Identify Sub-Optimal I/O
	Requests}\label{identify-io-calls}

We propose the following rules for applications to follow when issuing I/O requests to a particular SSD. Requests violating these rules are considered sub-optimal.

\begin{itemize}[leftmargin=*]
	\item \textbf{\textit{\underline{Rule 1}}}: \textit{Issue write requests that are multiples of the minimum desirable write request size}. Requests not obeying this rule either cause write amplification, or require more flash memory for storing logical-to-physical address mappings.
	\item \underline{\textbf{\textit{Rule 2}}}: \textit{Issue read requests of chunk size at hot locations whenever possible}. Hot locations in the logical address space provide significantly lower latencies, and the application should use this advantage if it can.
	\item \underline{\textbf{\textit{Rule 3}}}: \textit{Issue write requests aligned with stripe boundaries, preferably of stripe size}. Overwriting stripes completely is desirable, as any existing data and address mappings can be invalidated without fetching additional flash pages. Also, unaligned requests can disturb the regularity of hot locations (discussed further in Rule 4).
	\item \underline{\textit{\textbf{Rule 4}}}: \textit{Do not issue unaligned write requests of chunk size}. The distribution of chunks over channels determines where hot locations occur in the logical address space. Issuing write requests not aligned with chunks can destroy the regularity of hot locations.
	\item \revision{\underline{\textbf{\textit{Rule 5}}}: \textit{Issue write requests such that the number of flash pages modified are minimum.} For instance, write requests smaller than the flash page size will internally be padded up to a page, and thus require at least a single flash page. However, a small write request spanning two flash pages will require modifying both the pages, causing greater write amplification than necessary, and should be avoided.}
\end{itemize}

It should be noted that these rules help with maximizing the performance of the \textit{SSD alone}. However, the requirements of the application also need to be considered for an overall improvement in performance. For instance, it would be incorrect to conclude that the database engine should always issue an I/O of 64KB (stripe size) instead of say, 16KB. Doing so might entail more I/O time than necessary and could degrade the overall performance.

\subsubsection{The Benchmark Experiment}\label{benchmark-exp}

% The benchmark experiment described in this section is similar to SQLite4's benchmarking of its backend library~\cite{}. However, informed by previous work~\cite{}, we perform operations on a non-empty database instead. This experiment enables us to perform required measurements, such as recording I/O calls using \textit{strace}~\cite{}, measuring insert/select operation throughput, etc.

%	We run a benchmark experiment to record the I/O calls issued by a database engine for subsequent analysis using the above rules.

%	To evaluate a database engine using the rules described above, we run a benchmark experiment and record the I/O calls issued. 

We run a benchmark experiment and record the I/O calls issued by the database engine for subsequent analysis using the above rules. \revision{This experiment helps isolate the insert/select operation throughput of the database engine as a measure of its performance.} The experiment starts with an initial database containing 10 million key-value pairs in a single table. The key and value sizes are 32-byte and 100-byte respectively, and the initial size of the data is about 1.2GB. The experiment involves a single client running multiple iterations, with each iteration containing the following two phases:

\begin{enumerate}[leftmargin=*,noitemsep]
	\item Insert 50,000 new key-value pairs into the database in a random order.
	\item Run 50,000 select queries generated randomly on the set of keys present in the database.
\end{enumerate}

The size of the database increases by about 6MB (50,000 $\times$ 132B) during an iteration. The same workload has been run in all cases by using a fixed random seed. All the select operations are run in the same transaction, whereas the number of insert operations per transaction varies (details regarding this have been specified wherever applicable). 

This experiment is similar to SQLite's benchmarking of its backend library~\cite{lsmBenchmark}. However, informed by previous work~\cite{complexBenchmarking}, we perform operations on a non-empty database instead. Required measurements (like measuring insert/select operation throughput, recording I/O calls using \textit{strace}~\cite{strace}, etc.) are made during the experiment. 

% This experiment is similar to SQLite4's benchmarking of its backend library~\cite{}. However, informed by previous work~\cite{}, we run Insert and Select operations on a non-empty database.

% (PostgreSQL~\cite{}, InnoDB~\cite{}, Oracle DB~\cite{}, MS SQL Server~\cite{}, etc.)
\begin{figure}
	\centering
	\subfloat[\revision{Write requests of sizes 64KB and 128KB are made aligned with a 64KB block (rel. offset 0). These correspond to updates to database pages.}]{
		\includegraphics[scale=0.35]{figures/combined_btree_writes.png}
		\label{rollback-db-writes}
	}
	\hspace{3mm}
	\subfloat[\revision{Aligned read requests of size 64KB to the database pages are made. The remaining small requests are issued by SQLite3 to access its database header fields.}]{
		\includegraphics[scale=0.35]{figures/combined_btree_reads.png}
		\label{rollback-db-reads}
	}
	\vspace{-0.4em}
	\caption{\revision{\textbf{I/O profile of SQLite3 and MariaDB B$^+$-Tree index files during an iteration of the benchmark experiment for a B$^+$-Tree page size of 64KB. Pages are laid out contiguously in the index file, resulting in aligned requests that are multiples of 64KB. Both the databases violate Rule 2, as read requests are not issued to hot locations on SSD-S.}}}
	\label{rollback-db}
\end{figure}

\subsubsection{Analyzing the I/O behavior of B$^+$-Tree Indices}\label{analyzing-btree}

\revision{We study the I/O calls issued by SQLite3 and MariaDB to their primary index database files, to find any sub-optimal requests violating the rules (\S\ref{identify-io-calls}) on SSD-S. In both of these systems, the primary index file is structured as a B$^+$-Tree~\cite{sqliteFileFormat,innodb_btree}, and is divided into \textit{database pages}. Each database page corresponds to a node in the B$^+$-tree (Fig. \ref{fig:db_file_original_layout}), and the leaf nodes contain data rows.}

% (corresponding parameters summarized in Table \ref{ssds})
\revision{We investigate the I/O behavior of both the database engines for a B$^+$-Tree (database) page size of 64KB.} This matches the stripe size of most of our SSDs, which will be useful for a more comprehensive discussion involving the proposed rules. A single iteration of the benchmark experiment (\S\ref{benchmark-exp}) has been run with each insert operation in a separate transaction. \revision{Both database engines have been run in their default journaling modes (i.e, rollback journaling for SQLite3, and undo/redo logging in MariaDB w/InnoDB).}

\revision{Fig. \ref{rollback-db-writes} shows the write requests made by both database engines to their corresponding primary index files. We see that all the write requests are issued at aligned offsets, and are a multiple of the stripe size of SSD-S (64KB). Thus, none of the rules have been violated while issuing write requests.}

\revision{Fig. \ref{rollback-db-reads} shows the read requests issued to the B$^+$-tree index file by both the engines. The read requests of size 64KB at aligned offsets correspond to accessing pages from the index file. These requests violate Rule 2, as they are not issued to hot locations on SSD-S. The smaller read requests of size 100B and 4B are issued by SQLite3 to its database header. These requests are much smaller than a flash page and will cause read amplification. MariaDB doesn't issue any small read requests to its B$^+$-Tree database file.}

%SQLite3 has two journaling modes, and we apply the rules to both of them while running on SSD-S and SSD-T respectively as an example. The internal parameters of these SSDs are summarized in Table \ref{ssds}.

% We will be investigating the I/O behavior of SQLite3 for a database page size of 64KB. A single iteration of the benchmark experiment has been run, with each insert operation in its own separate transaction. SQLite3 has two journaling modes, and we apply the rules . As an example, we apply the rules assuming that SQLite3 is running on SSD-S and SSD-T respectively. The internal parameters of these SSDs have been summarized in Table \ref{ssds}.

\subsubsection{Analyzing the I/O Behavior of Log Files}\label{analyzing-logs}

%	\item \textit{{Rollback Journaling on SSD-S}}: This is the default journaling mode of SQLite3. The I/O requests to the database file are of interest to us, as the rollback journal is deleted immediately on commit. 
	
%	We see that all the write requests (Fig. \ref{rollback-db-writes}) are issued at aligned offsets, and are a multiple of the stripe size of SSD-S (64KB). Thus, none of the rules have been violated by the write requests.

\revision{We consider the logging behavior of SQLite3 and MariaDB on SSD-T. We have studied SQLite3 in its write-ahead logging (WAL) mode\footnote{\revision{SQLite3 in the rollback journal mode issues a mix of small and large writes to the log, similar to the WAL mode (see Fig. \ref{wal-log-writes}). However, we only study the WAL file as a representative example.}}~\cite{walsqlite3}, whereas we run MariaDB in its default mode involving undo/redo logging.}

\revision{Fig. \ref{wal-log-writes} show SQLite3's write requests to the WAL file. The 64KB requests correspond to writing dirty database pages to the log, and the smaller write requests of 24B (which violate Rule 1) are for writing the log frame headers (Fig. \ref{fig:wal_file_original}). Both these requests are increasingly unaligned with stripe boundaries, and violate Rule 3. All read requests (Fig. \ref{wal-log-reads}) are of size 64KB, and are increasingly offset into the stripe boundary. These requests are not issued at a 1KB boundary, and will cause read amplification inside the SSD.}
	
%The frame header causes all write and read requests (Fig. \ref{wal-log-reads}) of size 64KB to dirty pages to become increasingly offset with respect to the stripe boundary. These requests are not issued at a 1KB boundary, and will cause read/write amplification inside the SSD.}

	
%	\textit{Write-Ahead Logging (WAL) on SSD-T}: SQLite3 also supports write-ahead logging~\cite{walsqlite3}, where updates are first recorded in a separate log file and later checkpointed to the database file.
	
	
	\begin{figure}
		\centering
		\subfloat[Two types of write requests are issued: 24B requests for frame headers, and 64KB requests to write dirty database pages to the log.]{
			\includegraphics[scale=0.35]{figures/wal_log_writes.png}
			\label{wal-log-writes}
		}
		\hspace{3mm}
		\subfloat[Read requests of size 64KB are issued to dirty database pages (size 64KB) during checkpointing. Note that requests are unaligned.]{
			\includegraphics[scale=0.35]{figures/wal_log_reads.png}
			\label{wal-log-reads}
		}
		\vspace{-0.4em}
		\caption{\textbf{I/O profile of the SQLite3 WAL log file in WAL mode during an iteration of the benchmark experiment for a B$^+$-tree page size of 64KB. The log file is organized in frames, where a frame contains a header (24B) and a dirty page (64KB). Rules 1 \& 3 are violated by the write requests on SSD-T.}}
		\label{wal-log}
	\end{figure}
	
%	Fig. \ref{wal-log-writes} shows the write requests issued to the WAL log file. The 64KB requests correspond to writing dirty database pages to the log, and the smaller write requests of 24B are for writing the log frame headers (Fig. \ref{fig:wal_file_original}). Both of these requests are increasingly offset in a stripe (64KB) and violate Rule 3. Additionally, requests to the log frame headers are much smaller than the minimum desirable request size (64KB), and thus violate Rule 1.
	
%	All read requests (Fig. \ref{wal-log-reads}) are of size 64KB, and are increasingly offset with respect to the stripe boundary. These requests are not issued at a 1KB boundary, and will cause read amplification inside the SSD.

\revision{Compared to SQLite3, MariaDB has multiple log files to provide MVCC (undo logs), ensure crash recovery (redo logs) , avoid broken pages (doublewrite buffer), and provide log shipping to replicas (the binary log). These logs are contained in different tablespace files described in Fig. \ref{innodb-logs}, and the I/O requests to these files are discussed below.}
\begin{enumerate}[leftmargin=*,nolistsep]
	\item \revision{\textbf{\textit{The System Tablespace (ibdata)}}: Write requests of size 64KB aligning with stripe boundaries are issued, and none of the rules are violated\footnote{\revision{Rule 2 would have been violated on SSD-S, but not on SSD-T as its hot locations are at offset group 0. This file's layout is similar to the B$^+$-Tree index file (Fig.~\ref{fig:db_file_original_layout}). However, we do not recommend applying the technique \textit{use-hot-locations} to this file (see \S\ref{hot-locs-mariadb-perf}).}}.}
	\item \revision{\textbf{\textit{The Redo Log (ib\_logfile)}}: Write requests of size 512B are issued at offsets aligning with 512B boundary (thus contained in a single flash page). Rules 1 \& 3 are violated.}
	\item \revision{\textbf{\textit{The Binary Log (\{hostname\}-bin)}}: Small write requests of varying sizes at varying offsets are issued to this file. Rules 1, 3, and 5 are violated.}
\end{enumerate}

%The system tablespace file (\textit{ibdata1}) contains the undo logs and doublewrite buffer, and all write requests to this file are of size 64KB (stripe size of SSD-S) at aligned offsets. Thus, none of the rules are violated for this file. The Redo Log file has write requests of size 512B, violating Rules 1 and 3.
	
\begin{figure}
%	\vspace{0.5em}
	\centering
	\subfloat[\revision{Write requests to the system tablespace file are multiples of 64KB (stripe size for SSD-S) aligning with internal stripes, and don't violate any rules. The write requests to the redo log are of size 512B (aligned with 512B boundaries), and violate Rules 1 \& 3. The binary log on the other hand contains small write requests of varying sizes, which violate Rules 1, 3, and 5.}]{
		\includegraphics[scale=0.45]{figures/innodb_writes.png}
		\label{innodb-log-writes}
	}
	\vspace{-0.6em}
	\caption{\revision{\textbf{Write profile of MariaDB/InnoDB logs. The logs are contained in three files: (1) the System Tablespace file contains the undo log, doublewrite buffer, and the change buffer, (2) the Redo Log, and (3) the Binary Log for database replication. Read requests to these files follow a similar pattern.}}}
	\label{innodb-logs}
\end{figure}
	
% \noindent\underline{Rollback journaling on SSD-S}: First, we study the default rollback journaling mode~\cite{} of SQLite3. The I/O calls to the database file is of interest to us, as the rollback journal is deleted immediately after commit. Figures \ref{rollback-db-writes} and \ref{rollback-db-reads} show the read and write requests made to the database file. We observe three groups of read requests.

% Figure \ref{rollback-db-writes} shows the write requests issued to the database file. There are two groups of write requests, of size 64KB and 128KB, issued at relative offset 0. These requests do not violate any of the rules for SSD-S.

% The first group is comprised of requests of size 64Kb issued at relative offset 0. These requests are to the pages in the database file. These requests violate Rule 2, as they are not issued at good locations of SSD-S. The remaining requests are to the database header and file change counter, at relative offset 0-byte and 24-byte respectively. These requests violate Rule 1, as they are much smaller than the minimum desired size for SSD-S (16KB).

% \vspace{8pt}
% \noindent\underline{Write-Ahead-Logging (WAL) on SSD-T}: SQLite3 also supports write-ahead logging, where updates are first recorded into a separate log file and later checkpointed to the database file. The WAL log file is of interest to us, as the I/O behavior to the database file is similar to the case of rollback journaling.

% Figure \ref{wal-log-writes} shows the write issued to the WAL log file. There are two groups of write requests. The first group of requests is of size 64KB, which correspond to writing updated versions of database pages to the WAL log. These requests are increasingly offset into a 64KB block, and violate rule 3. The next group consists of requests of size 24-byte, which correspond to the log frame header (described further in Section 3.3). These requests violate rule 1, as they are smaller than 64KB.

% Figure \ref{wal-log-reads} shows the read requests issued to the WAL log file. All requests are of size 64KB. As SSD-T has no good locations, these requests do not violate any of the rules.

\begin{figure}
	\vspace{-0.6em}
	\subfloat[The original layout of the database file. Pages are laid out contiguously, aligning with 64KB chunks. Read and write requests are issued to addresses at offset group 0.]{
		\includegraphics[scale=0.43]{figures/db_file_original_layout.pdf}
		\label{fig:db_file_original_layout}
	}
	
	\vspace{-0.4em}
	\subfloat[The modified layout of the database file. All database pages are offset by 32KB, such that read requests to pages are issued to the 32KB offset group which are the hot locations for SSD-S. Write requests continue to align with a 64KB boundary to retain the internal chunk pattern (this is ensured by \textit{fsync}, see \S\ref{hot-locs-sqlite3-perf}).]{
		\includegraphics[scale=0.4]{figures/db_file_modified_layout.pdf}
		\label{fig:db_file_modified_layout}
	}
	\vspace{-0.4em}
	\caption{\revision{\textbf{\textit{use-hot-locations} on SSD-S. In both SQLite3 and MariaDB, the original layout of the B$^+$-Tree database file contains contiguous aligned pages of size 64KB. Hot locations on SSD-S can be utilized if the pages are offset by 32KB. Write requests to pages need to be modified to satisfy Rule 3.}}}
	\label{fig:use-good-locations}
%		\vspace{-.5em}
\end{figure}

\begin{figure}[H]
		\vspace{-0.5em}
	\centering
	\subfloat[\revision{The original layout of the InnoDB binary log file containing entries of varying sizes. Each entry internally requires the SSD to write a single flash page. However, entries spanning multiple flash pages (shown in red), will cause greater write amplification, as they will require modifying two flash pages instead.}]{
		\includegraphics[scale=0.37]{figures/bin_log_original.png}
		\label{fig:bin_log_original}
	}
	\vspace{-0.1em}
	\subfloat[\revision{The modified layout of the InnoDB binary log file. Entries spanning multiple flash pages are offset to align with the next page boundary. This results in a small varying amount of unused space at the end of each flash page, but reduces the write amplification caused by these entries to a single flash page.}]{
		\includegraphics[scale=0.37]{figures/bin_log_modified.png}
		\label{fig:bin_log_modified}
	}
	\vspace{-0.7em}
	\caption{\revision{\textbf{\textit{contain-write-in-flash-page} on SSD-T (flash page size 4KB). The MariaDB/InnoDB binary log file has been modified to eliminate log entries spanning over multiple flash pages. This reduces the write-amplification caused by the database engine.}}}
	\label{fig:contain-write-in-flash-page}
\end{figure}

\subsection{Techniques to Optimize Performance}\label{propose}

Having studied the I/O behavior of SQLite3 and MariaDB, we now propose techniques to improve their performance by eliminating sub-optimal I/O patterns. This is achieved by examining the data-structures used and making modifications to them to obtain the desired I/O behavior, \revision{while also considering the database engine's performance}. We propose the following techniques:

\begin{figure}
	%	\vspace*{1em}
	\centering
	\subfloat[The original layout of the WAL log file. The file has multiple frames, each with a frame header (24B) and a dirty page (64KB). As the log frame is not a multiple of stripe size (64KB), read/write requests become increasingly unaligned and violate Rule 3 (Fig. \ref{wal-log}).]{
		\includegraphics[scale=0.4]{figures/wal_file_original.pdf}
		\label{fig:wal_file_original}
	}
	
	%	\vspace*{1ex}
	\vspace{-0.4em}
	\subfloat[The modified layout of the WAL log file. The frame header is a small amount of memory, and can be included in the database page without reducing the capacity of the page by much. The new frame size is 64KB, which is equal to the stripe size. The log header of 32B is stored in a separate file to ensure that the log frames align with stripe boundaries. Writing the file header also causes write amplification, and is a one-time unavoidable cost.]{
		\includegraphics[scale=0.48]{figures/wal_file_modified_new.pdf}
		\label{fig:wal_file_modified}
	}
	\vspace{-0.4em}
	\caption{\textbf{\textit{write-aligned-stripes} on SSD-T. The SQLite3 WAL log file originally contains frames of size 64KB+24B. We include the 24B frame header in the page, to issue write requests of stripe size.}}
	\label{fig:write-stripes}
\end{figure}

\begin{enumerate}[leftmargin=*,nolistsep]
	\item {\textbf{\textit{use-hot-locations} on SSD-S}: Fig. \ref{fig:db_file_original_layout} shows the original layout of the B$^+$-Tree database file of both SQLite3 and MariaDB, where database pages align with internal stripes of SSD-S. This violates Rule 2 (see Fig. \ref{rollback-db-reads}), as read requests are issued at stripe boundaries instead of the hot locations (32KB offset group on SSD-S). To place the pages at hot locations, we offset them by 32KB in the modified layout of the file (Fig. \ref{fig:db_file_modified_layout}). However, in order to comply with Rule 3, write requests should continue to align with stripe boundaries, as shown in Fig. \ref{fig:db_file_modified_layout}. This technique is ineffective on the remaining SSDs as their hot locations are at offset group 0 (Rule 2 isn't violated).}
	\item {\textbf{\textit{write-aligned-stripes} on SSD-T}: The SQLite3 WAL file (Fig.~\ref{fig:wal_file_original}) has a 32B header followed by multiple \textit{frames}, each of which has a 24B frame header and a 64KB dirty page. These small header fields result in write amplification, as well as make the read/write requests to the dirty pages increasingly unaligned, thus violating Rules 1 \& 3 (Fig. \ref{wal-log}). We propose including the frame header at the end of the database page (Fig. \ref{fig:wal_file_modified}), and writing the WAL header (of 32B) to a separate file. This eliminates all violations of rules on SSD-T, as shown in Fig.~\ref{fig:wal_file_modified}. This technique will be effective on SSD-S and SSD-M as well, as they have the same stripe size as SSD-T.}
	\item \revision{\textbf{\textit{contain-write-in-flash-page} on SSD-T}: The MariaDB redo log and binary log both violate Rules 1 \& 3 (Fig.~\ref{innodb-logs}), as the requests are small and unaligned. However, issuing larger write requests would increase the latency of  commit operation, and degrade the DB engine's performance. Additionally, the binary log also violates Rule 5, as shown in Fig. \ref{fig:bin_log_original}. This violation can be eliminated by modifying the layout of the binary file as in Fig. \ref{fig:bin_log_modified}, where entries spanning multiple flash pages are offset to align with the next page boundary. This technique will also be effective on SSD-M, with a flash page size of 4KB.}
%		The MariaDB binary log violates Rules 1, 3, and 5 . Fig. \ref{fig:bin_log_original} shows the original layout of the binary file, where entries of varying sizes corresponding to different transactions are recorded sequentially. In our benchmark experiment, each}
\end{enumerate}

%The SQLite3 WAL log consists of a file header of size 32B, followed by one or more \textit{frames} (Fig. \ref{fig:wal_file_original}). Each frame contains a 24B frame header and a dirty page of size 64KB. We find that the log frames become increasingly offset in a stripe on SSD-T as they are not a multiple of 64KB. This causes the write requests to the frame headers and dirty pages in the log to become unaligned and violate Rule 3 (Fig. \ref{wal-log}). Additionally, the write requests to the frame headers (24B) are much smaller than a flash page, and will cause write amplification inside the SSD.

%In order to eliminate these undesirable I/O requests, we recommend issuing aligned write requests of stripe size to the log file. This can be accomplished on SSD-T (and the remaining SSDs as well) by including the log frame header in the database page as shown in Fig. \ref{fig:wal_file_modified}. A small amount of space (24B) is reserved at the end of the page for the frame header, and this does not reduce the capacity of the page by much. The log header of 32B is written to a separate file to ensure the alignment of frames with stripe boundaries. With this modified layout, all read/write requests to the log file are of stripe size and none of the rules are violated.

%The remaining SSDs have a chunk size of 4KB, with hot locations at offset group $0$. Thus, using this method on the remaining SSDs would not require changing the layout of the database file, as the B-Tree pages would already be present at hot locations.

% Informed by the sub-optimal I/O patterns found in the database engine (\S\ref{analyzing-sqlite3}), we now propose rules to improve its performance by eliminating such requests. This is achieved by examining the data-structures used by the database engine, and making modifications to them to obtain the desired I/O characteristics.

% Having studied the I/O patterns of a database engine using the described rules (\S\ref{identify-io-calls}), the next step is to propose methods to improve the performance of the database by eliminating sub-optimal I/O requests.

% To obtain an overall improvement in performance, the requirements of the database engine need to be considered along with the characteristics of the SSD it is running on. In this section, we propose methods to improve SQLite3's performance on SSD-S (\S\ref{method-use-hot-locations}) and SSD-T (\S\ref{method-write-stripes}). This is achieved by examining the data-structures used by the database engine, and making modifications to them to obtain the desired I/O characteristics.

% We use the learnt characteristics and parameters (Table \ref{ssds}) to make an informed decision regarding an application's operation.
% Use the learnt parameters to make an informed decision regarding an application's parameter choices.

%\subsubsection{use-hot-locations for B-Tree Pages}\label{method-use-hot-locations}
%
%As the name suggests, we propose using hot locations for storing B-Tree pages. Fig. \ref{fig:db_file_original_layout} shows the default layout of the SQLite3 database file consisting of contiguous B-Tree pages of size 64KB. Other databases such as PostgreSQL~\cite{postgres} with a B-Tree storage engine also have a file layout similar to Fig. \ref{fig:db_file_original_layout}.
%
%We first consider how to apply this method on SSD-S. When running in rollback journaling mode on SSD-S, we find that the read requests violate Rule 2 (Fig. \ref{rollback-db}) as they are not issued to hot locations on SSD-S (32KB offset group). The read requests correspond to accessing pages from the database file, which are present at offset group 0 in the original file layout. Thus, for read requests to be issued to hot locations, the database pages themselves need to be present at hot locations, i.e, \textit{the pages need to be offset by 32KB on SSD-S}. This requires modifying the layout of the database file as shown in Fig. \ref{fig:db_file_modified_layout}.

%With the modified layout, all database pages are offset by 32KB in the logical address space, and the first 32KB of the database file is unused. However, any write requests to database pages cannot be issued directly as they would be unaligned with the stripe boundary and violate Rule 3. To keep hot locations intact, multiple aligned write requests need to be issued while updating pages as shown in Fig. \ref{fig:db_file_modified_layout}.


%\subsubsection{write-aligned-stripes to the SQLite3 WAL log}\label{method-write-stripes}

\begin{figure*}
	\centering
	\subfloat[Select and Insert operation throughput over the iterations in a single run of the benchmark experiment \revision{with every insert operation in a separate transaction}. Total 100 iterations are executed with 50,000 select and insert operations issued in each iteration. \revision{For select(insert) operations, we see that the performance \textit{use-hot-locations} is consistently higher(lower) compared to the original. The average increase(decrease) in throughput is 30.4\%(15.2\%) over all the iterations. The loss in throughput of insert operations is caused by the additional \textit{fsync} (Fig.~\ref{fig:db_file_modified_layout})}.]{
		\includegraphics[scale=0.27]{figures/samsung_combined_benchmark_results.png}
		\label{fig:sqlite3_iterations}
	}
	\hspace{4mm}
	\subfloat[Select and Insert operation throughput over multiple runs of the benchmark experiment with varying granularity of transactions in the insert phase. The gain/loss in throughput during each run has been indicated. For select operations, we obtain an almost constant improvement, with a median increase of 29.2\%. For insert operations, as we increase the number of insert operations/transaction over the runs, the overhead of the additional \textit{fsync} call becomes amortized and is compensated by the benefit of faster seek time. The loss in insert throughput falls under 2\% from 500 insert operations/transaction onwards.]{
		\includegraphics[scale=0.3]{figures/select-insert-sqlite3-combined.png}
		\label{fig:sqlite3_hot_locs_runs}
	}
	%     \subfloat[Text]{
	% 		\includegraphics[scale=0.27]{insert_iterations.png}
	% 		\label{fig:insert_throughput_iterations}
	% 	}
	% 	\hspace{2mm}
	% 	\subfloat[Text]{
	% 		\includegraphics[scale=0.27]{insert_transactions.png}
	% 		\label{fig:insert_throughput_transactions}
	% 	}
	% 	\label{fig:write-stripes}
	\vspace{-0.4em}
	\caption{\textbf{\revision{The performance of SQLite3 with \textit{use-hot-locations} on SSD-S.} The B$^+$-Tree index file is modified such that pages are stored at hot locations (Fig. \ref{fig:db_file_modified_layout}). This leads to a reduction in latency while accessing pages, and a median increase of 29.2\% in select operation throughput as a result. \revision{The overhead of the additional \textit{fsync} (see Fig.~\ref{fig:db_file_modified_layout} and \S\ref{hot-locs-sqlite3-perf}) leads to a 15\% decrease in throughput of insert operations, but is compensated by faster seek time as we increase the number of insert operations per transaction.}}}
	\label{fig:hot-locs-sqlite3-perf}
\end{figure*}

%  This can be improved by including the WAL frame header within the database page, without sacrificing much on the capacity of the page.


% \footnote{One might argue that the new layout of the WAL log file (Fig. \ref{fig:wal_file_modified}) violates Rule 2 on SSD-S. However, WAL log frames are read sequentially at the time of checkpoint, and the benefit of hot locations is superseded by prefetching performed inside the SSD}.

% We use SQLITE\_TESTCTRL\_RESERVE~\cite{} to do this.

% On SSD-T, we would like to avoid the small writes of 24B to the WAL log file. Figure \ref{fig:wal_file_original} shows the format of the WAL log file. The log file is divided into frames, where each frame consists of a header of 24b and a database page of 64KB. Data is written to the log file in frames, which consists of a 24b write followed by a 64KB write.

% These can potentially be avoided by including the frame header within the database page, as shown in Fig. \ref{fig:wal_file_modified}. This way, the size of the WAL log frame will be equal to the database page size of 64KB. Reserving 24B of space for WAL frame header does not reduce the database page capacity by much.

%\subsubsection{contain-write-in-flash-page in MariaDB Binary Log}\label{method-contain-writes-in-pages}
